RoMath: A Mathematical Reasoning Benchmark in Romanian

Mathematics has long been conveyed through natural language, primarily for human understanding. With the rise of mechanized mathematics and proof assistants, there is a growing need to understand informal mathematical text, yet most existing benchmarks focus solely on English, overlooking other languages. This paper introduces RoMath, a Romanian mathematical reasoning benchmark suite comprising three subsets: Baccalaureate, Competitions and Synthetic, which cover a range of mathematical domains and difficulty levels, aiming to improve non-English language models and promote multilingual AI development. By focusing on Romanian, a low-resource language with unique linguistic features, RoMath addresses the limitations of Anglo-centric models and emphasizes the need for dedicated resources beyond simple automatic translation. We benchmark several open-weight language models, highlighting the importance of creating resources for underrepresented languages. Code and datasets are be made available.

==> tables/bac-sota.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{llrr}
\toprule
                                             \textbf{Model} &      \textbf{Setting} &  \textbf{Acc.} &   \textbf{F$_1$} \\
\midrule
                   OpenLLM-Ro/RoLlama3-8b-Instruct &     0-shot &      0.50 & 0.67 \\
                   OpenLLM-Ro/RoLlama3-8b-Instruct &     5-shot &      0.23 & 0.38 \\
                   OpenLLM-Ro/RoLlama3-8b-Instruct & fine-tuned &      0.18 & 0.31 \\
      
                  OpenLLM-Ro/RoMistral-7b-Instruct &     0-shot &      0.50 & 0.66 \\
                  OpenLLM-Ro/RoMistral-7b-Instruct &     5-shot &      0.20 & 0.33 \\
                  OpenLLM-Ro/RoMistral-7b-Instruct & fine-tuned &      0.18 & 0.31 \\
        \midrule
  
                            Qwen/Qwen2-7B-Instruct &     0-shot &      0.40 & 0.57 \\
                            Qwen/Qwen2-7B-Instruct &     5-shot &      0.35 & 0.52 \\
                            Qwen/Qwen2-7B-Instruct & fine-tuned &      0.54 & 0.70 \\
                            
                  microsoft/Phi-3-mini-4k-instruct &     0-shot &      0.36 & 0.53 \\
                  microsoft/Phi-3-mini-4k-instruct &     5-shot &      0.18 & 0.31 \\
                  microsoft/Phi-3-mini-4k-instruct & fine-tuned &      0.25 & 0.40 \\
                  
               meta-llama/Meta-Llama-3-8B-Instruct &     0-shot &      0.34 & 0.51 \\
               meta-llama/Meta-Llama-3-8B-Instruct &     5-shot &      0.28 & 0.44 \\
               meta-llama/Meta-Llama-3-8B-Instruct & fine-tuned &      0.18 & 0.31 \\
        \midrule
               
                       Qwen/Qwen2-Math-7B-Instruct &     0-shot &      0.32 & 0.48 \\
                       Qwen/Qwen2-Math-7B-Instruct &     5-shot &      0.22 & 0.36 \\
                       Qwen/Qwen2-Math-7B-Instruct & fine-tuned &      0.48 & 0.65 \\
          
             deepseek-ai/deepseek-math-7b-instruct &     0-shot &      0.56 & 0.72 \\
             deepseek-ai/deepseek-math-7b-instruct &     5-shot &      0.57 & 0.72 \\
             deepseek-ai/deepseek-math-7b-instruct & fine-tuned &      0.29 & 0.44 \\

                   mistralai/Mathstral-7b-v0.1 &     0-shot &      0.30 & 0.46 \\
                   mistralai/Mathstral-7b-v0.1 &     5-shot &      0.26 & 0.41 \\
                   mistralai/Mathstral-7b-v0.1 & fine-tuned &      0.21 & 0.34 \\

        \midrule
              meta-llama/Meta-Llama-3-70B-Instruct &     0-shot &      0.25 & 0.40 \\
              meta-llama/Meta-Llama-3-70B-Instruct &     5-shot &      0.08 & 0.15 \\
              
              mistralai/Mixtral-8x7B-Instruct-v0.1 &     0-shot &      0.43 & 0.60 \\
              mistralai/Mixtral-8x7B-Instruct-v0.1 &     5-shot &      0.25 & 0.40 \\
\bottomrule
\end{tabular}
}
    \caption{Results for various open-weight LLMs on RoMath-Baccalaureate, under 0-shot, 5-shot and fine-tuned scenarios.}
    \label{tab:bac-sota}
\end{table}

==> tables/comps-sota.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{llrr}
\toprule
                \textbf{Model} &      \textbf{Setting} &  \textbf{Acc.} &   \textbf{F$_1$} \\
\midrule
                   OpenLLM-Ro/RoLlama3-8b-Instruct &     0-shot &      0.48 & 0.65 \\
                   OpenLLM-Ro/RoLlama3-8b-Instruct &     5-shot &      0.26 & 0.41 \\
    OpenLLM/Ro-RoLlama3-8b-Instruct & fine-tuned &      0.50 & 0.67 \\
    
                  OpenLLM-Ro/RoMistral-7b-Instruct &     0-shot &      0.44 & 0.61 \\
                  OpenLLM-Ro/RoMistral-7b-Instruct &     5-shot &      0.16 & 0.27 \\
     OpenLLM-Ro/RoMistral-7b-Instruct & fine-tuned &      0.36 & 0.53 \\
     
        \midrule
                            Qwen/Qwen2-7B-Instruct &     0-shot &      0.55 & 0.71 \\
                            Qwen/Qwen2-7B-Instruct &     5-shot &      0.30 & 0.47 \\
                            Qwen/Qwen2-7B-Instruct & fine-tuned &      0.48 & 0.65 \\
             
                  microsoft/Phi-3-mini-4k-instruct &     0-shot &      0.33 & 0.50 \\
                  microsoft/Phi-3-mini-4k-instruct &     5-shot &      0.20 & 0.34 \\
                  microsoft/Phi-3-mini-4k-instruct & fine-tuned &      0.41 & 0.58 \\
   
               meta-llama/Meta-Llama-3-8B-Instruct &     0-shot &      0.53 & 0.69 \\
               meta-llama/Meta-Llama-3-8B-Instruct &     5-shot &      0.25 & 0.40 \\
               meta-llama/Meta-Llama-3-8B-Instruct & fine-tuned &      0.33 & 0.49 \\
        \midrule
                       Qwen/Qwen2-Math-7B-Instruct &     0-shot &      0.55 & 0.71 \\
                       Qwen/Qwen2-Math-7B-Instruct &     5-shot &      0.29 & 0.45 \\
                       Qwen/Qwen2-Math-7B-Instruct & fine-tuned &      0.57 & 0.73 \\
        
             deepseek-ai/deepseek-math-7b-instruct &     0-shot &      0.59 & 0.74 \\
             deepseek-ai/deepseek-math-7b-instruct &     5-shot &      0.33 & 0.49 \\
             deepseek-ai/deepseek-math-7b-instruct & fine-tuned &      0.56 & 0.72 \\
   
                       mistralai/Mathstral-7b-v0.1 &     0-shot &      0.61 & 0.75 \\
                       mistralai/Mathstral-7b-v0.1 &     5-shot &      0.35 & 0.52 \\
                      mistralai/Mathstral-7b-v0.1 & fine-tuned &      0.56 & 0.71 \\
        \midrule
              meta-llama/Meta-Llama-3-70B-Instruct &     0-shot &      0.22 & 0.36 \\
              meta-llama/Meta-Llama-3-70B-Instruct &     5-shot &      0.09 & 0.16 \\
   
              mistralai/Mixtral-8x7B-Instruct-v0.1 &     0-shot &      0.60 & 0.75 \\
              mistralai/Mixtral-8x7B-Instruct-v0.1 &     5-shot &      0.25 & 0.40 \\
\bottomrule
\end{tabular}
}
    \caption{Results for various open-weight LLMs on RoMath-Competitions, under 0-shot, 5-shot and fine-tuned scenarios.}
    \label{tab:comps-sota}
\end{table}

==> tables/english-prediction-prompt.tex <==
\begin{table}[hbt!]
    \begin{tcolorbox}[
        enhanced,
        attach boxed title to top left={xshift=6mm,yshift=-3mm},
        colback=white,
        colframe=gray!20,
        colbacktitle=white,
        % title={\scriptsize Selected examples from RoMath},
        fonttitle=\bfseries\color{black},
        boxed title style={size=small,colframe=gray!20,rounded corners},
        rounded corners,
        ]
        \vspace{2mm}
        \small
    \{\\
        "role": "system",\\
        "content": """You are a high school student who is preparing for a math competition. Your role is to solve high school math problems and provide complete and correct solutions.
Problems that require proofs should be solved completely with all necessary intermediate steps. Problems that have a single final answer should be provided in a boxed format (`$\backslash$boxed\{\}`).
Mathematics should be written in LaTeX format to ensure the clarity and precision of the solutions. The LaTeX-formatted text should be delimited using the symbols `$\backslash$(` and `$\backslash$)`."""\\
    \},\\
    \# add few shot examples here: User => Problem statement, Assistant => Solution\\
    \{\\
        "role": "user",\\
        "content": """What is the solution to the following problem?\\

\{problem\_statement\}""",\\
    \}
    \end{tcolorbox}
    \caption{English prediction prompt.}
    \label{tab:english-prediction-prompt}
\end{table}

==> tables/sota-united.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{cllrr|rr|rr}
\toprule
            & & & \multicolumn{2}{c}{\textbf{Baccalaureate}} &  \multicolumn{2}{c}{\textbf{Competitions}} &  \multicolumn{2}{c}{\textbf{Synthetic}} \\
            &\textbf{Model} &      \textbf{Scenario} &  \textbf{Accuracy} &  \textbf{F1} &  \textbf{Accuracy} &  \textbf{F1} &   \textbf{Accuracy} &  \textbf{F1} \\
\midrule
       \multirow{6}{*}{\rotatebox{90}{\textbf{Romanian}}} & &     0-shot &        0.50 &  0.67 &        0.48 &  0.65 &      0.18 & 0.30 \\
      & OpenLLM-Ro/RoLlama3-8b-Instruct &     5-shot &        0.23 &  0.38 &        0.26 &  0.41 &      0.27 & 0.43 \\
       & & fine-tuned &        0.18 &  0.31 &        0.50 &  0.67 &      -- & -- \\
      \cmidrule{3-9}
      & &     0-shot &        0.50 &  0.66 &        0.44 &  0.61 &      0.16 & 0.27 \\
     & OpenLLM-Ro/RoMistral-7b-Instruct &     5-shot &        0.20 &  0.33 &        0.16 &  0.27 &      0.22 & 0.36 \\
      & & fine-tuned &        0.18 &  0.31 &        0.36 &  0.53 &      -- & -- \\
      \midrule
                \multirow{9}{*}{\rotatebox{90}{\textbf{General-Purpose}}} & &     0-shot &        0.40 &  0.57 &        0.55 &  0.71 &      0.29 & 0.45 \\
               & Qwen/Qwen2-7B-Instruct &     5-shot &        0.35 &  0.52 &        0.30 &  0.47 &      0.25 & 0.40 \\
                & & fine-tuned &        0.54 &  0.70 &        0.48 &  0.65 &      -- & -- \\
 \cmidrule{3-9}
      &&     0-shot &        0.36 &  0.53 &        0.33 &  0.50 &      0.07 & 0.14 \\
     &microsoft/Phi-3-mini-4k-instruct &     5-shot &        0.18 &  0.31 &        0.20 &  0.34 &      0.20 & 0.33 \\
      && fine-tuned &        0.25 &  0.40 &        0.41 &  0.58 &      -- & -- \\
     \cmidrule{3-9}
   &&     0-shot &        0.34 &  0.51 &        0.53 &  0.69 &      0.25 & 0.40 \\
  &meta-llama/Meta-Llama-3-8B-Instruct &     5-shot &        0.28 &  0.44 &        0.25 &  0.40 &      0.13 & 0.22 \\
   && fine-tuned &        0.18 &  0.31 &        0.33 &  0.49 &      -- & -- \\

 \midrule
           \multirow{9}{*}{\rotatebox{90}{\textbf{Math-Specialized}}} &&     0-shot &        0.32 &  0.48 &        0.55 &  0.71 &      0.27 & 0.43 \\
          &Qwen/Qwen2-Math-7B-Instruct &     5-shot &        0.22 &  0.36 &        0.29 &  0.45 &      0.21 & 0.35 \\
           && fine-tuned &        0.48 &  0.65 &        0.57 &  0.73 &      -- & -- \\
          \cmidrule{3-9}
 &&     0-shot &        0.56 &  0.72 &        0.59 &  0.74 &      0.21 & 0.35 \\
& deepseek-ai/deepseek-math-7b-instruct &     5-shot &        0.57 &  0.72 &        0.33 &  0.49 &      0.29 & 0.45 \\
 && fine-tuned &        0.29 &  0.44 &        0.56 &  0.72 &      -- & -- \\
\cmidrule{3-9}
           & &     0-shot &        0.30 &  0.46 &        0.61 &  0.75 &      0.36 & 0.53 \\
          &mistralai/Mathstral-7b-v0.1 &     5-shot &        0.26 &  0.41 &        0.35 &  0.52 &      0.13 & 0.22 \\
           && fine-tuned &        0.21 &  0.34 &        0.56 &  0.71 &      -- & -- \\

\midrule
 \multirow{4}{*}{\rotatebox{90}{\textbf{Large}}}& meta-llama/Meta-Llama-3-70B-Instruct &     0-shot &        0.25 &  0.40 &        0.22 &  0.36 &      0.10 & 0.19 \\
  &&     5-shot &        0.08 &  0.15 &        0.09 &  0.16 &      0.07 & 0.13 \\
         \cmidrule{3-9}
 &mistralai/Mixtral-8x7B-Instruct-v0.1 &     0-shot &        0.43 &  0.60 &        0.60 &  0.75 &      0.32 & 0.48 \\
  &&     5-shot &        0.25 &  0.40 &        0.25 &  0.40 &      0.24 & 0.38 \\
\bottomrule
\end{tabular}
}
    \caption{Results for various open-weight LLMs on RoMath-Baccalaureate, RoMath-Competitions and RoMath-Synthetic, under 0-shot, 5-shot and fine-tuned scenarios.}
    \label{tab:romath-sota}
\end{table}

==> tables/synthetic-sota.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{llrr}
\toprule
            \textbf{Model} &      \textbf{Setting} &  \textbf{Acc.} &   \textbf{F$_1$} \\
\midrule
      OpenLLM-Ro/RoLlama3-8b-Instruct & 0-shot &      0.18 & 0.30 \\
      OpenLLM-Ro/RoLlama3-8b-Instruct & 5-shot &      0.27 & 0.43 \\
     OpenLLM-Ro/RoMistral-7b-Instruct & 0-shot &      0.16 & 0.27 \\
     OpenLLM-Ro/RoMistral-7b-Instruct & 5-shot &      0.22 & 0.36 \\
     \midrule
               Qwen/Qwen2-7B-Instruct & 0-shot &      0.29 & 0.45 \\
               Qwen/Qwen2-7B-Instruct & 5-shot &      0.25 & 0.40 \\
               
     microsoft/Phi-3-mini-4k-instruct & 0-shot &      0.07 & 0.14 \\
     microsoft/Phi-3-mini-4k-instruct & 5-shot &      0.20 & 0.33 \\
  meta-llama/Meta-Llama-3-8B-Instruct & 0-shot &      0.25 & 0.40 \\
  meta-llama/Meta-Llama-3-8B-Instruct & 5-shot &      0.13 & 0.22 \\
    \midrule
          Qwen/Qwen2-Math-7B-Instruct & 0-shot &      0.27 & 0.43 \\
          Qwen/Qwen2-Math-7B-Instruct & 5-shot &      0.21 & 0.35 \\
deepseek-ai/deepseek-math-7b-instruct & 0-shot &      0.21 & 0.35 \\
deepseek-ai/deepseek-math-7b-instruct & 5-shot &      0.29 & 0.45 \\
          mistralai/Mathstral-7b-v0.1 & 0-shot &      0.36 & 0.53 \\
          mistralai/Mathstral-7b-v0.1 & 5-shot &      0.13 & 0.22 \\
    \midrule
 meta-llama/Meta-Llama-3-70B-Instruct & 0-shot &      0.10 & 0.19 \\
 meta-llama/Meta-Llama-3-70B-Instruct & 5-shot &      0.07 & 0.13 \\
 mistralai/Mixtral-8x7B-Instruct-v0.1 & 0-shot &      0.32 & 0.48 \\
 mistralai/Mixtral-8x7B-Instruct-v0.1 & 5-shot &      0.24 & 0.38 \\
\bottomrule
\end{tabular}
}
    \caption{Results for various open-weight LLMs on RoMath-Synthetic, under 0-shot and 5-shot scenarios.}
    \label{tab:synthetic-sota}
\end{table}
